Triboelectric Charging Model for Particles with Rough Surfaces

The triboelectric charging of particles depends on the contact area of the particle and the contacting surface. Even though the surface topology determines the real contact area, particle charging models do not account for surface roughness. In this paper, we combine contact mechanics and triboelectrification models to predict the charging of rough particles. First, a laser confocal microscope measured the statistical descriptors of polyethylene (PE) particles surface topology. Then, we descriptors particle surfaces by distributing spheroidal asperities on the smooth particle core until the surface roughness reaches the measured value. The Hertz contact mechanics model predicts the deformation of the asperity-covered particle and the resulting real contact area in dependence on impact velocity. Finally, we introduced the real contact area into the condenser model for triboelectric particle charging. The accuracy of the new model predictions was demonstrated by comparing it to a more complex surface reconstructions that account for the fractal surface topology. Furthermore, the model's predicted particle saturation charges agree well with our shaker experiments and with experimental data in the literature on the charging of plane surfaces. The developed triboelectric charging model for particles with rough surfaces is simple and requires only standard descriptors of the surface topology; thus, it suits large-scale simulations of electrifying powder flows.

==> Schematics.tex <==
\begin{tikzpicture}[scale=0.50]
    
  % \shade[ball color = gray!40, opacity = 0.4] (0,0) circle (2cm);
  % \draw (0,0) circle (5cm);
       \shade[ color = gray!40, opacity = 0.4,rotate=13] (2.9,2.7) arc (90:270:0.8 and 1);
    \shade[color = gray!40, opacity = 0.4,rotate=13] (2.9,0.7) arc (-90:90:1 and 1);
  \draw (-2,-2) arc (270:360:7 and 2);
  \draw (-2,-2) arc (180:90:2 and 7);
  \draw (0,5) arc (90:0:5 and 5);
  %\draw[dashed] (5,0) arc (0:90:5 and 1);
  \draw[dashed] (3,-1.3) arc (0:90:3 and 6.3);
  %\draw[dashed] (-1.6,2) arc (270:360:5.6 and 1);
  \fill[fill=black] (0,0) circle (1pt);
  \fill[fill=black] (2.45,2.3) circle (2pt);
  %\draw[dashed] (0,0 ) -- node[above]{$x$} (5,0);
  \draw[dashed,ultra thick,->] (0,0 )-- node[above]{$x$} (5,0);
  \draw[dashed,ultra thick,->] (0,0 ) -- node[above]{$y$}(-2,-2);
  \draw[dashed,ultra thick,->] (0,0 )-- node[left]{$z$} (0,5);
  \draw (0,0 ) --  node[above,sloped]{$r_p$} (2.45,2.3);
  \draw[dashed] (0,0 ) -- (3,-1.4);
  \draw [->](-1,-1) arc (270:315:3.5 and 1);
  \draw [<-](1.5,1.4) arc (45:78:3 and 6.3);
  \node at (1.2,2.5) [rotate=-30]{$\phi_i$};
  \node at (0.4,-1.2) [rotate=10]{$\theta_i$};

    \draw [rotate=13] (2.9,2.7) arc (90:270:0.8 and 1);
    \draw [dashed,rotate=13] (2.9,0.7) arc (-90:90:0.8 and 1);
    \draw [rotate=13] (2.9,0.7) arc (-90:90:1 and 1);
    \draw (2.45,2.3) --  node[above,sloped]{$r_i$} (1.65,2.3);
    
\end{tikzpicture}


==> Schematics3.tex <==
\begin{tikzpicture}[scale=1.5]
\draw[dashed] (0,0) arc (0:180:1 and 0.2);
\draw (-2,0) arc (180:360:1 and 0.2);
\draw[pattern=crosshatch, pattern color=gray!40]  (-1,0) ellipse (1 and 0.2);
\draw[] (0,0) arc (0:180:1 and 1);

\draw[dashed] (-0.15,0.5) arc (0:180:0.85 and 0.1);
\draw (-1.85,0.5) arc (180:360:0.85 and 0.1);

\draw
[
	decoration={
		coil,
		segment length = 3,
		amplitude = 4,
		aspect = 0.5,
		post length = 1,
		pre length = 1},
	decorate] (-1,0) -- ++(0,0.5);
 \draw
[
	decoration={
		coil,
		segment length = 3,
		amplitude = 4,
		aspect = 0.5,
		post length = 1,
		pre length = 1},
	decorate] (-1.5,0) -- ++(0,0.5);
 \draw
[
	decoration={
		coil,
		segment length = 3,
		amplitude = 4,
		aspect = 0.5,
		post length = 1,
		pre length = 1},
	decorate] (-1.25,0) -- ++(0,0.5);
 \draw
[
	decoration={
		coil,
		segment length = 3,
		amplitude = 4,
		aspect = 0.5,
		post length = 1,
		pre length = 1},
	decorate] (-0.75,0) -- ++(0,0.5);
 \draw
[
	decoration={
		coil,
		segment length = 3,
		amplitude = 4,
		aspect = 0.5,
		post length = 1,
		pre length = 1},
	decorate] (-0.5,0) -- ++(0,0.5);
\draw[pattern=grid, pattern color=gray!40]  (-1,0.5) ellipse (0.85 and 0.1);

  \node at (-1,-0.1) [rotate=0]{$A_{i,\mathrm{max}}$};
  \node at (-0.75,0.75) [rotate=0]{$A_{c,i}$};


  \draw[] (-1,1) -- (0.4,1);
  \draw[] (-0.15,0.5) -- (0.1,0.5);
  \draw[] (0,0) -- (0.4,0);
  \draw[<->] (0.1,1) -- node[right]{$\delta_i$} (0.1,0.5);
  \draw[<->] (0.4,1) -- node[right]{$r_i$} (0.4,0);
  \draw[<->] (0.1,0) -- node[right]{$d$} (0.1,0.5); %sim: original formulation
  
  \draw[] (-1,0.5) -- (-1.85,0.5);
  \node at (-1.5,0.65) [rotate=0]{$r_{c,i}$};



\end{tikzpicture}
